PODNet: Pooled Outputs Distillation for Small-Tasks Incremental Learning

Lifelong learning has attracted much attention, but existing works still struggle to fight catastrophic forgetting and accumulate knowledge over long stretches of incremental learning. In this work, we propose PODNet, a model inspired by representation learning. By carefully balancing the compromise between remembering the old classes and learning new ones, PODNet fights catastrophic forgetting, even over very long runs of small incremental tasks --a setting so far unexplored by current works. PODNet innovates on existing art with an efficient spatial-based distillation-loss applied throughout the model and a representation comprising multiple proxy vectors for each class. We validate those innovations thoroughly, comparing PODNet with three state-of-the-art models on three datasets: CIFAR100, ImageNet100, and ImageNet1000. Our results showcase a significant advantage of PODNet over existing art, with accuracy gains of 12.10, 6.51, and 2.85 percentage points, respectively. Code is available at https://github.com/arthurdouillard/incremental_learning.pytorch

==> tables/ablation_initialincrement.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}lcccccc@{}}
 \toprule
 Initial task size & 10 & 20 & 30 & 40 & 50\\
 \midrule
iCaRL \cite{rebuffi2017icarl}     & 40.97 & 41.28 & 43.38 & 44.35 & 44.20\\
BiC \cite{bias_correction}        & 41.58 & \tbd  & 42.27 & 45.18 & 47.09\\
UCIR (NME) \cite{hou2019ucir} & 42.33 & 40.81 & 46.80 & 46.71 & 48.57\\
UCIR (CNN) \cite{hou2019ucir} & 43.25 & 41.69 & 47.85 & 47.51 & 49.30\\
PODNet (NME) & \textbf{45.09} & \textbf{49.03} & \textbf{55.30} & \textbf{57.89} & \textbf{61.07}\\
PODNet (CNN)& \textbf{44.95} & \textbf{47.68} & \textbf{52.88} & \textbf{55.42} & \textbf{57.84}\\
\bottomrule
\end{tabular}
\caption{Effect of the initial task size on the models performance. Results from CIFAR100 with incremental steps of 1 classes, we report the average incremental accuracy.}
\label{tab:ablation_initialincrement}
\end{table}

==> tables/ablation_mmnca.tex <==
%\begin{table}[t]{\textwidth}
%\centering
%\begin{tabular}{@{}lcccc@{}}
% \toprule
% Classifier & Nb modes & NME & CNN\\
% \midrule
% Cosine     & ---  & 58.89 & 56.38   \\
% MM-NCA     & 1    & 60.52 & 56.8    \\
% MM-NCA     & 5    & 60.88 & 57.55   \\
% MM-NCA     & 10   & 61.00 & 57.84   \\
% MM-CCE     & 10   & \tbd  & \tbd    \\
%\bottomrule
%\end{tabular}
%\caption{Comparison of different classifiers used at the end of STILL.}
%\label{tab:ablation_clf}
%\end{table}

\begin{table}[t]{\textwidth}
\centering
\begin{tabular}{@{}lcccc@{}}
 \toprule
 Classifier & IOD-flat & IOD-spatial & CNN\\
 \midrule
 Cosine     & \OK      & \OK         & \tbd   \\
 Cosine    & \OK       &             & \tbd   \\
 LSC        & \OK      &             & \tbd    \\
 LSC        & \OK      & \OK         & \tbd    \\
\bottomrule
\end{tabular}
\caption{Comparison of STILL with and without the Local Similarity Classifier (LSC)}
\label{tab:ablation_clf}
\end{table}

==> tables/quantitative.tex <==
% \begin{table*}[t]
% \begin{subtable}[t]{\textwidth}
% \centering
% \begin{tabular}{@{}lcccc@{}}
%  \toprule
%   & 25 steps & 10 steps & 5 steps\\
%  \midrule
%  Images per step & 1,000 & 2,500 & 5,000\\
%  \midrule[1.5pt]
%  iCaRL \cite{icarl}     & 50.59 $\pm$ 1.29  & 53.77 $\pm$ 1.42  & 58.07 $\pm$ 0.72\\
%  BiC \cite{bias_correction} & 48.96 $\pm$ 1.26 & 53.21 $\pm$ 1.25  & 56.85 $\pm$ 0.56\\
%  UCIR (NME) \cite{ucir}     & 56.82 $\pm$ 0.23 & 60.83 $\pm$ 0.85 & 63.63 $\pm$ 1.07\\
%  UCIR (CNN) \cite{ucir}     & 57.23 $\pm$ 0.67 & 61.22 $\pm$ 0.85 & 64.01 $\pm$ 1.12\\
%  STILL & \textbf{61.58 $\pm$ 0.64} & \textbf{63.31 $\pm$ 0.73} & \textbf{64.66 $\pm$ 0.76}\\
%  \bottomrule
% \end{tabular}

% \caption{Average Incremental Accuracy on CIFAR100 on 3 random orders.}
% \label{tab:avginc_cifar100}
% \end{subtable}
% \vspace{1em}

% \begin{subtable}[t]{0.5\textwidth}
% \centering
% \begin{tabular}{@{}lcccc@{}}
%  \toprule
%   & 25 steps & 10 steps & 5 steps\\
%  \midrule
%  Images per step: & 2,500 & 6,400 & 12,800\\
%  \midrule[1.5pt]
%  iCaRL \cite{icarl}         & 54.56 & 60.90  & 65.56 \\
%  BiC \cite{bias_correction} & 59.65 & 65.14 & 68.97\\
%  UCIR (NME) \cite{ucir}     & 60.81 & 65.83 & 69.07\\
%  UCIR (CNN) \cite{ucir}     & 62.94 & 67.82 & 71.04\\
%  STILL                      & \textbf{63.33} & \textbf{70.30} &  \textbf{73.13}\\
%  \bottomrule
% \end{tabular}
% \caption{Avg Incremental Accuracy on ImageNet100.}
% \label{tab:avginc_imagenet100}
% \end{subtable}
% \hfill
% \begin{subtable}[t]{0.45\textwidth}
% \centering
% \begin{tabular}{@{}lccc@{}}
%  \toprule
%   & 20 steps & 10 steps\\
%  \midrule
%  Images per step: & 2,500      & 5,000\\
%  \midrule[1.5pt]
%  UCIR (NME) \cite{ucir}     & 37.14  & 40.32 \\
%  UCIR (CNN) \cite{ucir}     & \textbf{38.24}  & 41.12 \\
%  STILL                      & 37.20    & \textbf{42.56} \\
%  \bottomrule
% \end{tabular}
% \caption{Avg Incremental Accuracy on TinyImageNet-200.}
% \label{tab:avginc_tinyimagenet200}
% \end{subtable}

% \caption{Quantitative results on CIFAR100, ImageNet100, and TinyImagenet200.}
% \label{tab:quantitative}
% \end{table*}







\begin{table*}[t]
\centering
\begin{tabular}{@{}l|ccc|ccc|cc@{}}
 \toprule
 & \multicolumn{3}{c|}{CIFAR100} & \multicolumn{3}{c|}{Imagenet100} & \multicolumn{2}{c}{TinyImageNet200} \\
 %\cmidrule(l{0pt}r{4pt}){2-4} \cmidrule(l{4pt}r{4pt}){5-7} \cmidrule(l{4pt}r{4pt}){8-9}
  & 25 steps & 10 steps & 5 steps & 25 steps & 10 steps & 5 steps & 20 steps & 10 steps\\
 \multicolumn{1}{r|}{Images per step} & 1,000 & 2,500 & 5,000& 2,500 & 6,400 & 12,800 & 2,500      & 5,000\\
 \midrule
 iCaRL \cite{icarl}     & 50.60 $\pm$ 1.06  & 53.78 $\pm$ 1.16  & 58.08 $\pm$ 0.59& 54.56 & 60.90  & 65.56 & --- & ---\\
 BiC \cite{bias_correction} & 48.96 $\pm$ 1.03 & 53.21 $\pm$ 1.01  & 56.86 $\pm$ 0.46& 59.65 & 65.14 & 68.97 & --- & ---\\
 UCIR (NME) \cite{ucir}     & 56.82 $\pm$ 0.19 & 60.83 $\pm$ 0.70 & 63.63 $\pm$ 0.87& 60.81 & 65.83 & 69.07& 37.14  & 40.32 \\
 UCIR (CNN) \cite{ucir}     & 57.57 $\pm$ 0.23 & 61.22 $\pm$ 0.69 & 64.01 $\pm$ 0.91& 62.94 & 67.82 & 71.04& \textbf{38.24}  & 41.12 \\
 STILL & \textbf{61.58 $\pm$ 0.52} & \textbf{63.31 $\pm$ 0.60} & \textbf{64.66 $\pm$ 0.62}& \textbf{63.33} & \textbf{70.30} &  \textbf{73.13}& 37.20    & \textbf{42.56} \\
 \bottomrule
\end{tabular}

\caption{Average incremental accuracy, STILL \textit{vs.} state of the art. We run experiments thrice (random class orders) on CIFAR100 and report averages $\pm$ standard deviations. An experimental run has a starting task with half the classes, and then a number of additional tasks indicated in the steps, with the remaining classes evenly divided among them.}
\label{tab:quantitative_all}
\end{table*}



==> tables/v2tables.tex <==
\begin{table*}[t]
\begin{subtable}[t]{\textwidth}
\centering
\begin{tabular}{@{}lcccc@{}}
 \toprule
 \# of images per steps & 500 & 1,000 & 2,500 & 5,000\\
 \midrule[1.5pt]
 Algorithm & 50 steps  & 25 steps & 10 steps & 5 steps\\
 \midrule
 iCaRL \cite{icarl}     & 44.20 $\pm$ 1.20 & 50.59 $\pm$ 1.29  & 53.77 $\pm$ 1.42  & 58.07 $\pm$ 0.72\\
 BiC \cite{bias_correction} & 47.09 $\pm$ 1.81 & 48.96 $\pm$ 1.26 & 53.21 $\pm$ 1.25  & 56.85 $\pm$ 0.56\\
 UCIR (NME) \cite{ucir}     & 48.57 $\pm$ 0.45 & 56.82 $\pm$ 0.23 & 60.83 $\pm$ 0.85 & 63.63 $\pm$ 1.07\\
 UCIR (CNN) \cite{ucir}     & 49.30 $\pm$ 0.39 & 57.23 $\pm$ 0.67 & 61.22 $\pm$ 0.85 & 64.01 $\pm$ 1.12\\
 STILL & \textbf{57.11 $\pm$ 1.19} & \textbf{61.58 $\pm$ 0.64} & \textbf{63.31 $\pm$ 0.73} & \textbf{64.66 $\pm$ 0.76}\\
 STILL v2 (NME + Spatial) & \tmp{60.47} & \tbd & \tbd & \tbd \\ 
 \bottomrule
\end{tabular}

\caption{Average Incremental Accuracy on CIFAR100 on 3 random orders.}
\label{tab:avginc_cifar100}
\end{subtable}
\vspace{1em}

\begin{subtable}[t]{0.5\textwidth}
\centering
\begin{tabular}{@{}lcccc@{}}
 \toprule
  \# of images per steps & 1,200 & 2,500 & 6,400 & 12,800\\
 \midrule
 Algorithm & 50 steps & 25 steps & 10 steps & 5 steps\\
 \midrule[1.5pt]
 iCaRL \cite{icarl}         & \tmp{54.97} & 54.56 & 60.90  & 65.56 \\
 BiC \cite{bias_correction} & \tmp{46.49} & 59.65 & 65.14 & 68.97\\
 UCIR (NME) \cite{ucir}     & 55.44 & 60.81 & 65.83 & 69.07\\
 UCIR (CNN) \cite{ucir}     & 57.25 & 62.94 & 67.82 & 71.04\\
 STILL                      & 53.89 & 63.33 & 70.30 &  73.13\\
 STILL v2 (CNN)             & \textbf{\tmp{60.98}}  & \textbf{\tmp{66.57}} & \textbf{\tmp{73.14}} & \textbf{\tmp{75.82}}\\
 \bottomrule
\end{tabular}
\caption{Avg Incremental Accuracy on ImageNet100.}
\label{tab:avginc_imagenet100}
\end{subtable}
\hfill
\begin{subtable}[t]{0.45\textwidth}
\centering
\begin{tabular}{@{}lccc@{}}
 \toprule
 \# of images per steps & 1,000       & 2,500      & 5,000\\
 \midrule
 Algorithm                  & 50 steps & 20 steps & 10 steps\\
 \midrule[1.5pt]
 UCIR (NME) \cite{ucir}     & 32.09     & 37.14  & 40.32 \\
 UCIR (CNN) \cite{ucir}     & 33.01     & 38.24  & 41.12 \\
 STILL                      & 26.31      & 37.2    & \textbf{42.56} \\
 STILL v2 (CNN)                   & \tmp{9.62}      & \tmp{34.25}     & \tmp{37.44} \\
 STILL v2 (NME)                   & \tmp{33.22}      & \tmp{40.61}      & \tmp{44.36} \\
 \bottomrule
\end{tabular}
\caption{Avg Incremental Accuracy on TinyImageNet-200.}
\label{tab:avginc_tinyimagenet200}
\end{subtable}

\caption{Quantitative results on CIFAR100, ImageNet100, and TinyImagenet200.}
\label{tab:quantitative}
\end{table*}


\begin{table}[tb]
\begin{center}
\begin{tabular}{@{}lccccc@{}}
 \toprule
 Algorithm& 25 steps & 10 steps & 5 steps\\
 \midrule
 iCaRL \cite{icarl}         & --- & 46.72  & 51.36\\
 BiC \cite{bias_correction} & --- & --- & --- \\
 UCIR (NME) \cite{ucir}     & 57.02 & 59.92 & 61.56\\
 UCIR (CNN) \cite{ucir}     & 58.43 & 61.28 & 64.34\\
 STILL v2                   & \tbd & \tbd & \tbd\\
 \bottomrule
\end{tabular}
\end{center}
\caption{Avg Incremental Accuracy on ImageNet1000}
\label{tab:avginc_imagenet1000}
\end{table}

\begin{table}[tb]
\begin{center}
\begin{tabular}{@{}lccccc@{}}
 \toprule
 Variant & Factor & Scheduled Factor & Score\\
 \midrule
 Spatial Corr & --- & 1             &  \tmp{55.54}\\
 Depth Percent & --- & 1 & \tmp{56.07}\\
SpatialChannels & --- & 8 & \tmp{56.16}\\
MaxPoolChannels & --- & 4 & \tmp{56.83}\\
Base    & 5      & ---              &  57.21\\
MMD        & --- & 55  & \tmp{57.80}\\
Percent & ---    & 6                &  \tmp{58.57}\\
Percent (10/1/1/1) & --- & 6 & \tmp{58.99}\\
SpatialPercent (10/1/1/1) & --- & 4 & \tmp{59.64}\\
MaxPoolSpatial & --- & 6 & \tmp{60.19}\\
Spatial & ---    & 5                &  \textbf{\tmp{60.47}}\\
 \bottomrule
\end{tabular}
\end{center}
\caption{Comparison RAD variant on CIFAR100, inc1}
\label{tab:avginc_imagenet1000}
\end{table}




\begin{table}[tb]
\begin{tabular}{@{}ccccc@{}}
 \toprule
 Classif. & \multicolumn{2}{c}{Distillation} & Spread. & \\
 \cmidrule(l{0pt}r{4pt}){1-1} \cmidrule(l{4pt}r{4pt}){2-3} \cmidrule(l{4pt}r{4pt}){4-4}
 MM-NCA & LF & RAD & DMR & Score \\
 \midrule
 \OK &     &     &       & 41.56 \\
 \OK & \OK &     &       & \tmp{48.78 1order}  \\
 \OK &  &  \OK   &       & \tmp{51.04 1order}  \\
 \OK & \OK & \OK &       & \tmp{57.21 1order} \\
 \bottomrule
\end{tabular}
\caption{Comparison of the performance of the model when disabling parts of the complete STILL loss.}
\label{tab:ablation_inc}
\end{table}
%
\begin{table}[tb]
\begin{tabular}{@{}lc@{}}
 \toprule
 Distillation Loss      & Score \\
 \midrule
 None                   & \tmp{48.78 1order}    \\
 Perceptual Features \cite{percetual_losses_johnson16}    & \tmp{49.74 1order}   \\
 GradCam \cite{learning_without_memorizing_gradcam} & \tmp{50.45 1order}\\
 Perceptual Style \cite{percetual_losses_johnson16}      & \tmp{51.01 1order}   \\
 RAD \cite{attention_residual_distillation}                   & \tmp{57.11 1order}  \\
 RAD Spatial & \textbf{\tmp{60.47 1order}}\\
 \bottomrule
\end{tabular}
\caption{Comparison of perceptual losses.}
\label{tab:ablation_perceptual}

\caption{Ablation studies performed on CIFAR100 with 50 steps. We report the average incremental accuracy.}

\end{table}

